Approximating Edit Distance in Truly Subquadratic Time: Quantum and MapReduce

The edit distance between two strings is defined as the smallest number of insertions, deletions, and substitutions that need to be made to transform one of the strings to another one. Approximating edit distance in subquadratic time is "one of the biggest unsolved problems in the field of combinatorial pattern matching". Our main result is a quantum constant approximation algorithm for computing the edit distance in truly subquadratic time. More precisely, we give an $O(n^{1.858})$ quantum algorithm that approximates the edit distance within a factor of $7$. We further extend this result to an $O(n^{1.781})$ quantum algorithm that approximates the edit distance within a larger constant factor. Our solutions are based on a framework for approximating edit distance in parallel settings. This framework requires as black box an algorithm that computes the distances of several smaller strings all at once. For a quantum algorithm, we reduce the black box to \textit{metric estimation} and provide efficient algorithms for approximating it. We further show that this framework enables us to approximate edit distance in distributed settings. To this end, we provide a MapReduce algorithm to approximate edit distance within a factor of $3$, with sublinearly many machines and sublinear memory. Also, our algorithm runs in a logarithmic number of rounds.

==> figs/windowscomp1.tex <==
\begin{figure*}[h!]
\begin{center}
\includegraphics[scale=0.7]{figs/fig4.pdf}
\end{center}
\caption{The substitution operations and intact characters are shown by edges from $s_1$ to $s_2$. Dashed edges represent those with one covered endpoint. Dotted edges represent those that are remained at the end of the iteration.}
\label{fig:wincomp1}
\end{figure}

\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.7]{figs/fig5.pdf}
\end{center}
\caption{Dotted rectangles represent $v_i$'s and $v'_i$'s. Dashed rectangles represent shifted windows that are in $W_1$ or $W_2$. Dashed lines represent edges that are left outside of windows after shifting.}
\label{fig:wincomp1}
\end{figure*}
